Animated Logic: Correct Functional Conversion to Conjunctive Normal Form

We present an approach to obtain formally verified implementations of classical Computational Logic algorithms. We choose the Why3 platform because it allows to implement functions in a style very close to the mathematical definitions, as well as it allows a high degree of automation in the verification process. As proof of concept, we present a mathematical definition of the algorithm to convert propositional formulae to conjunctive normal form, implementations in WhyML (the Why3 language, very similar to OCaml), and proofs of correctness of the implementations. We apply our proposal on two variants of this algorithm: one in direct-style and another with an explicit stack structure. Being both first-order versions, Why3 processes the proofs naturally.

==> appendicesBackup.tex <==
\newpage

\section{Código OCaml extraído a partir da implementação WhyML}
\label{appendix:codigoocaml}

\begin{why3}
type ident = string

type formula =
  | FVar of ident
  | FConst of bool
  | FAnd of formula * formula
  | FOr of formula * formula
  | FImpl of formula * formula
  | FNeg of formula

type formula_wi =
  | FVar_wi of ident
  | FConst_wi of bool
  | FAnd_wi of formula_wi * formula_wi
  | FOr_wi of formula_wi * formula_wi
  | FNeg_wi of formula_wi
  
let rec impl_free (phi: formula) : formula_wi =
  begin match phi with
  | FNeg phi1 -> FNeg_wi (impl_free phi1)
  | FOr (phi1, phi2) -> FOr_wi ((impl_free phi1), (impl_free phi2))
  | FAnd (phi1, phi2) -> FAnd_wi ((impl_free phi1), (impl_free phi2))
  | FImpl (phi1, phi2) -> FOr_wi ((FNeg_wi (impl_free phi1)), (impl_free phi2))
  | FConst phi1 -> FConst_wi phi1
  | FVar phi1 -> FVar_wi phi1
  end

let rec nnfc (phi: formula_wi) : formula_wi =
  begin match phi with
  | FNeg_wi (FNeg_wi phi1) -> nnfc phi1
  | FNeg_wi (FAnd_wi (phi1, phi2)) -> FOr_wi ((nnfc (FNeg_wi phi1)), (nnfc (FNeg_wi phi2)))
  | FNeg_wi (FOr_wi (phi1, phi2)) -> FAnd_wi ((nnfc (FNeg_wi phi1)), (nnfc (FNeg_wi phi2)))
  | FOr_wi (phi1, phi2) -> FOr_wi ((nnfc phi1), (nnfc phi2))
  | FAnd_wi (phi1, phi2) -> FAnd_wi ((nnfc phi1), (nnfc phi2))
  | phi1 -> phi1
  end

let rec distr (phi1: formula_wi) (phi2: formula_wi) : formula_wi =
  begin match (phi1, phi2) with
  | (FAnd_wi (phi11, phi12), phi21) ->
    let o = distr phi12 phi21 in let o1 = distr phi11 phi21 in FAnd_wi (o1, o)
  | (phi11, FAnd_wi (phi21, phi22)) ->
    let o = distr phi11 phi22 in let o1 = distr phi11 phi21 in FAnd_wi (o1, o)
  | (phi11, phi21) -> FOr_wi (phi11, phi21)
  end

let rec cnfc (phi: formula_wi) : formula_wi =
  begin match phi with
  | FOr_wi (phi1, phi2) -> let o = cnfc phi2 in let o1 = cnfc phi1 in distr o1 o
  | FAnd_wi (phi1, phi2) ->
    let o = cnfc phi2 in let o1 = cnfc phi1 in FAnd_wi (o1, o)
  | phi1 -> phi1
  end

let t (phi: formula) : formula_wi = cnfc (nnfc (impl_free phi))
\end{why3}

\newpage

\section{Contagem de Construtores}
\label{appendix:size}

\begin{why3}
function size (phi: formula_wi) : int 
= match phi with
  | FVar_wi _ | FConst_wi _ -> 1
  | FNeg_wi phi -> 1 + size phi
  | FAnd_wi phi1 phi2 | FOr_wi phi1 phi2 ->
        1 + size phi1 + size phi2
end
\end{why3}

\section{Lema auxiliar para a contagem dos construtores}
\label{appendix:construtores}

\begin{why3}
let rec lemma size_nonneg (phi: formula_wi)
  variant { phi }
  ensures { size phi >= 0 }
= match phi with
  | FVar_wi _ | FConst_wi _ -> ()
  | FNeg_wi phi -> size_nonneg phi
  | FAnd_wi phi1 phi2 | FOr_wi phi1 phi2 ->
        size_nonneg phi1; size_nonneg phi2
end
\end{why3}

\section{Versão em CPS}
\label{appendix:cps}

\begin{why3} 
let rec impl_free_cps (phi: formula) (k: formula_wi -> 'a ) : 'a
 = match phi with
  | FNeg phi1 -> impl_free_cps phi1 (fun con -> k (FNeg_wi con))
  | FOr phi1 phi2 -> impl_free_cps phi1 (fun con -> impl_free_cps phi2 (fun con1 -> k (FOr_wi con con1)))
  | FAnd phi1 phi2 -> impl_free_cps phi1 (fun con -> impl_free_cps phi2 (fun con1 -> k (FAnd_wi con con1)))
  | FImpl phi1 phi2 -> impl_free_cps phi1 (fun con -> impl_free_cps phi2 (fun con1 -> k (FOr_wi (FNeg_wi con) con1)))
  | FConst phi -> k (FConst_wi phi)
  | FVar phi -> k (FVar_wi phi)
end

let impl_free_main (phi: formula) : formula_wi
= impl_free_cps phi (fun x -> x)

let rec nnfc_cps (phi: formula_wi) (k: formula_wi -> 'a) : 'a
= match phi with
  | FNeg_wi (FNeg_wi phi1) -> nnfc_cps phi1 (fun con -> k con)
  | FNeg_wi (FAnd_wi phi1 phi2) -> nnfc_cps (FNeg_wi phi1) (fun con -> nnfc_cps (FNeg_wi phi2) (fun con1 -> k (FOr_wi con con1)))
  | FNeg_wi (FOr_wi phi1 phi2) -> nnfc_cps (FNeg_wi phi1) (fun con -> nnfc_cps (FNeg_wi phi2) (fun con1 -> k (FAnd_wi con con1)))
  | FOr_wi phi1 phi2 -> nnfc_cps phi1 (fun con -> nnfc_cps phi2 (fun con1 -> k (FOr_wi con con1)))
  | FAnd_wi phi1 phi2 -> nnfc_cps phi1 (fun con -> nnfc_cps phi2 (fun con1 -> k (FAnd_wi con con1)))
  | phi -> k (phi)
end

let nnfc_main (phi: formula_wi) : formula_wi
= nnfc_cps phi (fun x -> x)

let rec distr_cps (phi1 phi2: formula_wi) (k: formula_wi -> 'a) : 'a
= match phi1, phi2 with
  | FAnd_wi phi11 phi12, phi2 -> distr_cps phi11 phi2 (fun con -> distr_cps phi12 phi2 (fun con1 -> k (FAnd_wi con con1)))
  | phi1, FAnd_wi phi21 phi22 -> distr_cps phi1 phi21 (fun con -> distr_cps phi1 phi22 (fun con1 -> k (FAnd_wi con con1)))
  | phi1,phi2 -> k (FOr_wi phi1 phi2)
    end

let distr_main (phi1 phi2: formula_wi) : formula_wi
= distr_cps phi1 phi2 (fun x -> x)

let rec cnfc_cps (phi: formula_wi) (k: formula_wi -> 'a) : 'a
= match phi with
  | FOr_wi phi1 phi2 -> cnfc_cps phi1 (fun con -> cnfc_cps phi2 (fun con1 -> distr_cps con con1 k))
  | FAnd_wi phi1 phi2 -> cnfc_cps phi1 (fun con -> cnfc_cps phi2 (fun con1 -> k (FAnd_wi con con1)))
  | phi -> k (phi)
end

let cnfc_main (phi: formula_wi) : formula_wi
= cnfc_cps phi (fun x -> x)
\end{why3}

\newpage

\section{Correção das funções em CPS}
\label{appendix:provacps}

\subsection{NNFC}

\begin{why3}
let rec nnfc_cps (phi: formula_wi) (k: formula_wi -> 'a) : 'a
  variant { size phi }
  ensures { result = k (nnfc phi) }
= ...
    
let nnfc_main (phi: formula_wi) : formula_wi
  ensures { forall v. eval_wi v phi = eval_wi v result } 
  ensures { wf_negations_of_literals result }
= nnfc_cps phi (fun x -> x)
\end{why3}

\subsection{CNFC}

\begin{why3}
let rec cnfc_cps (phi: formula_wi) (k: formula_wi -> 'a) : 'a
  requires{ wf_negations_of_literals phi }
  variant { phi }
  ensures{ result = k (cnfc phi)}
= ...

let cnfc_main (phi: formula_wi) : formula_wi
  requires{ wf_negations_of_literals phi }
  ensures{ forall v. eval_wi v phi = eval_wi v result }
  ensures{ wf_negations_of_literals result }
  ensures{ wf_conjunctions_of_disjunctions result}
= cnfc_cps phi (fun x -> x)
\end{why3}

\newpage

\section{Versão Desfuncionalizada}
\label{appendix:desfun}


\subsection{Tipos}
\begin{why3} 
type impl_kont =
  | KImpl_Id
  | KImpl_Neg impl_kont formula
  | KImpl_OrLeft formula impl_kont
  | KImpl_OrRight impl_kont formula_wi
  | KImpl_AndLeft formula impl_kont
  | KImpl_AndRight impl_kont formula_wi
  | KImpl_ImplLeft formula impl_kont
  | KImpl_ImplRight impl_kont formula_wi

type nnfc_kont =
  | Knnfc_id
  | Knnfc_negneg nnfc_kont formula_wi
  | Knnfc_negandleft formula_wi nnfc_kont
  | Knnfc_negandright nnfc_kont formula_wi
  | Knnfc_negorleft formula_wi nnfc_kont
  | Knnfc_negorright nnfc_kont formula_wi
  | Knnfc_andleft formula_wi nnfc_kont
  | Knnfc_andright nnfc_kont formula_wi
  | Knnfc_orleft formula_wi nnfc_kont
  | Knnfc_orright nnfc_kont formula_wi
    
type distr_kont =
  | KDistr_Id
  | KDistr_Left formula_wi formula_wi distr_kont
  | KDistr_Right distr_kont formula_wi
    
type cnfc_kont =
  | KCnfc_Id
  | KCnfc_OrLeft formula_wi cnfc_kont
  | KCnfc_OrRight cnfc_kont formula_wi
  | KCnfc_AndLeft formula_wi cnfc_kont
  | KCnfc_AndRight cnfc_kont formula_wi
\end{why3}

\subsection{Função Impl\_Free}

\begin{why3}
let rec impl_free_desf_cps (phi: formula) (k: impl_kont) : formula_wi
= match phi with
  | FNeg phi1 -> impl_free_desf_cps phi1 (KImpl_Neg k phi1)
  | FOr phi1 phi2 -> impl_free_desf_cps phi1 (KImpl_OrLeft phi2 k)
  | FAnd phi1 phi2 -> impl_free_desf_cps phi1 (KImpl_AndLeft phi2 k)
  | FImpl phi1 phi2 -> impl_free_desf_cps phi1 (KImpl_ImplLeft phi2 k)
  | FConst phi -> impl_apply (FConst_wi phi) k
  | FVar phi -> impl_apply (FVar_wi phi) k
end

with impl_apply (phi: formula_wi) (k: impl_kont) : formula_wi
= match k with
  | KImpl_Id -> phi
  | KImpl_Neg k phi1 -> impl_apply (FNeg_wi phi) k
  | KImpl_OrLeft phi1 k -> impl_free_desf_cps phi1 (KImpl_OrRight k phi)
  | KImpl_OrRight k phi2 -> impl_apply (FOr_wi phi2 phi) k
  | KImpl_AndLeft phi1 k -> impl_free_desf_cps phi1 (KImpl_AndRight k phi)
  | KImpl_AndRight k phi2 -> impl_apply (FAnd_wi phi2 phi) k
  | KImpl_ImplLeft phi1 k -> impl_free_desf_cps phi1 (KImpl_ImplRight k phi)
  | KImpl_ImplRight k phi2-> impl_apply (FOr_wi (FNeg_wi phi2) phi) k
end

let rec impl_desf_main (phi:formula) : formula_wi
= impl_free_desf_cps phi KImpl_Id
  

\end{why3}

\subsection{Função NNFC}

\begin{why3}
let rec nnfc_desf_cps (phi: formula_wi) (k: nnfc_kont) : formula_wi
= match phi with
  | FNeg_wi (FNeg_wi phi1) -> nnfc_desf_cps phi1 (Knnfc_negneg k phi1)
  | FNeg_wi (FAnd_wi phi1 phi2) -> nnfc_desf_cps (FNeg_wi phi1) (Knnfc_negandleft phi2 k)
  | FNeg_wi (FOr_wi phi1 phi2) -> nnfc_desf_cps (FNeg_wi phi1) (Knnfc_negorleft phi2 k)
  | FOr_wi phi1 phi2 -> nnfc_desf_cps phi1 (Knnfc_orleft phi2 k)
  | FAnd_wi phi1 phi2 -> nnfc_desf_cps phi1 (Knnfc_andleft phi2 k)
  | phi -> nnfc_apply phi k
end

with nnfc_apply (phi: formula_wi) (k: nnfc_kont) : formula_wi
= match k with
  | Knnfc_id -> phi
  | Knnfc_negneg k phi1 -> nnfc_apply phi k
  | Knnfc_negandleft phi1 k -> nnfc_desf_cps (FNeg_wi phi1) (Knnfc_negandright k phi)
  | Knnfc_negandright k phi2 -> nnfc_apply (FOr_wi phi2 phi) k
  | Knnfc_negorleft phi1 k -> nnfc_desf_cps (FNeg_wi phi1) (Knnfc_negorright k phi)
  | Knnfc_negorright k phi2 -> nnfc_apply (FAnd_wi phi2 phi) k
  | Knnfc_andleft phi1 k -> nnfc_desf_cps phi1 (Knnfc_andright k phi)
  | Knnfc_andright k phi2 -> nnfc_apply (FAnd_wi phi2 phi) k
  | Knnfc_orleft phi1 k -> nnfc_desf_cps phi1 (Knnfc_orright k phi)
  | Knnfc_orright k phi2 -> nnfc_apply (FOr_wi phi2 phi) k
end

let nnfc_desf_main (phi: formula_wi) : formula_wi
= nnfc_desf_cps phi Knnfc_id
\end{why3}

\subsection{Função Distr}

\begin{why3}
let rec distr_desf_cps (phi1 phi2: formula_wi) (k: wf_distr_kont) : formula_wi
= match phi1,phi2 with
  | FAnd_wi phi11 phi12, phi2 ->
        distr_desf_cps phi11 phi2 { distr_k = KDistr_Left phi12 phi2 k.distr_k }
  | phi1, FAnd_wi phi21 phi22 ->
        distr_desf_cps phi1 phi21 { distr_k = KDistr_Left phi1 phi22 k.distr_k }
  | phi1,phi2 -> distr_apply (FOr_wi phi1 phi2) k
end

with distr_apply (phi: formula_wi) (k: wf_distr_kont) : formula_wi
= match k.distr_k with
  | KDistr_Id -> phi
  | KDistr_Left phi1 phi2 k ->
        distr_desf_cps phi1 phi2 { distr_k = KDistr_Right k phi }
  | KDistr_Right k phi1 ->
        distr_apply (FAnd_wi phi1 phi) { distr_k = k }
end

let distr_desf_main (phi1 phi2: formula_wi) : formula_wi
= distr_desf_cps phi1 phi2 { distr_k = KDistr_Id }
\end{why3}

\subsection{Função CNFC}

\begin{why3}
let rec cnfc_desf_cps (phi: formula_wi) (k: wf_cnfc_kont) : formula_wi
= match phi with
  | FOr_wi phi1 phi2 ->
        cnfc_desf_cps phi1 { cnfc_k = KCnfc_OrLeft phi2 k.cnfc_k }
  | FAnd_wi phi1 phi2 ->
        cnfc_desf_cps phi1 { cnfc_k = KCnfc_AndLeft phi2 k.cnfc_k }
  | phi -> cnfc_apply phi k
end

with cnfc_apply (phi: formula_wi) (k: wf_cnfc_kont) : formula_wi
= match k.cnfc_k with
  | KCnfc_Id -> phi
  | KCnfc_OrLeft phi1 k ->
        cnfc_desf_cps phi1 { cnfc_k = KCnfc_OrRight k phi }
  | KCnfc_OrRight k phi2 ->
        cnfc_apply (distr_desf_cps phi2 phi { distr_k = KDistr_Id })
          { cnfc_k = k }
  | KCnfc_AndLeft phi1 k ->
        cnfc_desf_cps phi1 { cnfc_k = KCnfc_AndRight k phi }
  | KCnfc_AndRight k phi2 ->
        cnfc_apply (FAnd_wi phi2 phi) { cnfc_k = k }
end

let cnfc_desf_main (phi: formula_wi) : formula_wi
= cnfc_desf_cps phi { cnfc_k = KCnfc_Id }
\end{why3}

\newpage

\section{Correção das funções desfuncionalizadas}
\label{appendix:provadesfun}

\subsection{NNFC}

\begin{why3}
predicate nnfc_post (k: nnfc_kont) (phi result: formula_wi)
= match k with
  | Knnfc_id -> let x = phi in x = result
  | Knnfc_negneg k phi1 -> let neg = phi in nnfc_post k phi result
  | Knnfc_negandleft phi1 k -> let hl = phi in nnfc_post k (FOr_wi phi (nnfc (FNeg_wi phi1))) result
  | Knnfc_negandright k phi2 -> let hr = phi in nnfc_post k (FOr_wi phi2 hr) result
  | Knnfc_negorleft phi1 k -> let hl = phi in nnfc_post k (FAnd_wi phi (nnfc (FNeg_wi phi1))) result
  | Knnfc_negorright k phi2 ->let hr = phi in nnfc_post k (FAnd_wi phi2 hr) result
  | Knnfc_andleft phi1 k -> let hl = phi in nnfc_post k (FAnd_wi phi (nnfc phi1)) result
  | Knnfc_andright k phi2 -> let hr = phi in nnfc_post k (FAnd_wi phi2 hr) result
  | Knnfc_orleft phi1 k -> let hl = phi in nnfc_post k (FOr_wi phi (nnfc phi1)) result
  | Knnfc_orright k phi2 -> let hr = phi in nnfc_post k (FOr_wi phi2 hr) result
end
  
let rec nnfc_desf_cps (phi: formula_wi) (k: nnfc_kont) : formula_wi
  ensures{ nnfc_post k (nnfc phi) result }
= ...

with nnfc_apply (phi: formula_wi) (k: nnfc_kont) : formula_wi
  ensures{ nnfc_post k phi result }
= ...
\end{why3}

\subsection{CFNC}

\begin{why3}
predicate cnfc_post (k: cnfc_kont) (phi result: formula_wi)
= match k with
  | KCnfc_Id -> let x = phi in x = result
  | KCnfc_OrLeft phi1 k -> let hl = phi in cnfc_post k (distr hl (cnfc phi1)) result
  | KCnfc_OrRight k phi2 -> let hr = phi in cnfc_post k (distr phi2 hr) result
  | KCnfc_AndLeft phi1 k -> let hl = phi in cnfc_post k (FAnd_wi phi (cnfc phi1)) result
  | KCnfc_AndRight k phi2 -> let hr = phi in cnfc_post k (FAnd_wi phi2 hr) result
end
  
let rec cnfc_desf_cps (phi: formula_wi) (k: wf_cnfc_kont) : formula_wi
  requires{ wf_negations_of_literals phi }
  ensures{ cnfc_post k.cnfc_k (cnfc phi) result }
= ...

with cnfc_apply (phi: formula_wi) (k: wf_cnfc_kont) : formula_wi
  requires{ wf_negations_of_literals phi }
  requires { wf_conjunctions_of_disjunctions phi }
  ensures{ cnfc_post k.cnfc_k phi result }
= ...
\end{why3}

\subsection{Especificação da função Distr}
\begin{why3}
predicate wf_distr_kont (phi: distr_kont) 
= match phi with
  | KDistr_Id -> true
  | KDistr_Left phi1 phi2 k ->
        wf_negations_of_literals phi1 /\ wf_conjunctions_of_disjunctions phi1 /\
        wf_negations_of_literals phi2 /\ wf_conjunctions_of_disjunctions phi2 /\
        wf_distr_kont k
  | KDistr_Right k phi ->
        wf_negations_of_literals phi /\ wf_conjunctions_of_disjunctions phi /\ wf_distr_kont k
end

type wf_distr_kont = {
    distr_k: distr_kont;
} invariant { wf_distr_kont distr_k }
by { distr_k = KDistr_Id }
\end{why3}\textbf{}

\subsection{Especificação da função T desfuncionalizada}
\label{appendix:tdesf}

\begin{why3}
let t (phi: formula) : formula_wi
  ensures{ forall v. eval v phi = eval_wi v result }
  ensures{ wf_negations_of_literals result }
  ensures{ wf_conjunctions_of_disjunctions result }
= cnfc_desf_main(nnfc_desf_main(impl_desf_main phi))
\end{why3}

\clearpage

==> motivacao.tex <==
\section{Introdução}
\label{sec:motivation}

\myparagraphbf{Motivação:} Este artigo insere-se no projeto \texttt{FACTOR}\cite{factor}, que visa promover o uso do OCaml\cite{leroy2014ocaml} na comunidade académica de expressão portuguesa. Tendo como objetivos a implementação funcional de algoritmos clássicos de lógica computacional e linguagens formais, provas de correção ``automáticas" das mesmas e a execução passo-a-passo para a frente e para trás para ajudar a compreender os algoritmos a partir de exemplos.

Neste artigo pegamos no algoritmo que converte fórmulas proposicionais para a forma normal conjuntiva (FNC) e seguimos o programa proposto: implementação em WhyML\cite{filliatre2013why3} (uma linguagem da família ML que permite depois uma extração para código OCaml), realizamos a sua prova de correção e para suportar no futuro a execução passo-a-passo fazemos também uma implementação CPS\cite{sabry1993reasoning}, as dificuldades que nos deparamos na prova obrigou-nos a passar para a desfuncionalização. 

\myparagraphbf{Trabalho relacionado:} Existem livros clássicos que apresentam este algoritmo em pseudo-código não executável, temos por exemplo o conhecido livro ``Logic in Computer Science: Modelling and reasoning about systems'' \cite{huth2004logic}. A implementação destes algoritmos é uma peça fundamental para a aprendizagem e compreensão dos mesmos, no entanto esta não pode ser muito complexa e divergente das definições matemáticas, o que pode ser conseguido com linguagens funcionais como o OCaml.

\myparagraphbf{Contribuições:} A contribuição principal deste artigo é a apresentação e implementação funcional do algoritmo, juntamente com as provas em Why3\cite{filliatre2013why3} da versão direta e desfuncionalizada a partir de uma versão CPS.
